Online convex optimization for constrained control of linear systems using a reference governor

In this work, we propose a control scheme for linear systems subject to pointwise in time state and input constraints that aims to minimize time-varying and a priori unknown cost functions. The proposed controller is based on online convex optimization and a reference governor. In particular, we apply online gradient descent to track the time-varying and a priori unknown optimal steady state of the system. Moreover, we use a $\lambda$-contractive set to enforce constraint satisfaction and a sufficient convergence rate of the closed-loop system to the optimal steady state. We prove that the proposed scheme is recursively feasible, ensures that the state and input constraints are satisfied at all times, and achieves a dynamic regret that is linearly bounded by the variation of the cost functions. The algorithm's performance and constraint satisfaction is illustrated by means of a simulation example.

==> figures/Simulation_alpha.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\breite,
height=0.75\breite,
at={(0\breite,0\breite)},
scale only axis,
xmin=1,
xmax=100,
ymin=-0.0,
ymax=1.05,
xlabel={time steps $t$},
ylabel style={font=\color{white!15!black}},
ylabel={$\alpha$},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	1\\
2	1\\
3	1\\
4	1\\
5	1\\
6	1\\
7	1\\
8	1\\
9	1\\
10	1\\
11	1\\
12	1\\
13	1\\
14	1\\
15	1\\
16	1\\
17	1\\
18	1\\
19	1\\
20	1\\
21	1\\
22	1\\
23	1\\
24	1\\
25	1\\
26	1\\
27	1\\
28	1\\
29	1\\
30	1\\
31	0.110595703125\\
32	0.054595947265625\\
33	0.095550537109375\\
34	0.17608642578125\\
35	0.3189697265625\\
36	0.6973876953125\\
37	1\\
38	1\\
39	1\\
40	1\\
41	1\\
42	1\\
43	1\\
44	1\\
45	1\\
46	1\\
47	1\\
48	1\\
49	1\\
50	1\\
51	1\\
52	1\\
53	1\\
54	1\\
55	0.840179443359375\\
56	1\\
57	1\\
58	1\\
59	1\\
60	1\\
61	1\\
62	1\\
63	1\\
64	1\\
65	1\\
66	1\\
67	1\\
68	1\\
69	1\\
70	1\\
71	1\\
72	1\\
73	1\\
74	1\\
75	1\\
76	1\\
77	1\\
78	1\\
79	1\\
80	1\\
81	1\\
82	1\\
83	1\\
84	1\\
85	1\\
86	1\\
87	1\\
88	1\\
89	1\\
90	1\\
91	1\\
92	1\\
93	1\\
94	1\\
95	1\\
96	1\\
97	1\\
98	1\\
99	1\\
100	1\\
};

\end{axis}

\begin{axis}[%
width=1.227\breite,
height=0.92\breite,
at={(-0.16\breite,-0.101\breite)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%

==> figures/Simulation_u.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\breite,
height=0.75\breite,
at={(0\breite,0\breite)},
scale only axis,
xmin=1,
xmax=100,
ymin=-0.4,
ymax=0.2,
xlabel={time steps $t$},
ylabel style={font=\color{white!15!black}},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	0\\
2	-0.161680655065616\\
3	-0.247191965405639\\
4	-0.292726069809201\\
5	-0.3221445802988\\
6	-0.324203960120299\\
7	-0.324203970218803\\
8	-0.324203973129732\\
9	-0.32420397526987\\
10	-0.324203976726108\\
11	-0.324203977644951\\
12	-0.324203978185132\\
13	-0.324203978483872\\
14	-0.324203978642078\\
15	-0.324203740072803\\
16	-0.324203978138492\\
17	-0.324203978522645\\
18	-0.324203661432416\\
19	-0.324203804237188\\
20	-0.324203873659557\\
21	-0.324203912251722\\
22	-0.324203936104449\\
23	-0.324203951590514\\
24	-0.324203961720357\\
25	-0.324203968258315\\
26	-0.324203972389355\\
27	-0.324203974941278\\
28	-0.324203978109555\\
29	-0.324203978351329\\
30	-0.32420397850147\\
31	-0.282665305659938\\
32	-0.258382813882215\\
33	-0.21820526681522\\
34	-0.151238325391517\\
35	-0.0512922600756133\\
36	0.0975262381871583\\
37	0.162101942709097\\
38	0.162101929782529\\
39	0.162101913074666\\
40	0.162101989373046\\
41	0.162101989358861\\
42	0.162101989340027\\
43	0.162101989314362\\
44	0.162101989277922\\
45	0.162101989222998\\
46	0.1621019891338\\
47	0.162101988977103\\
48	0.16210198833143\\
49	0.162101987390957\\
50	0.162101985463763\\
51	0.162101981509989\\
52	0.162101973465523\\
53	0.162101957239027\\
54	0.162101923737667\\
55	0.104158614135126\\
56	0.0524863140092813\\
57	0.0265013741541692\\
58	0.00813002411993019\\
59	-0.00626828622750331\\
60	-0.0185707427329436\\
61	-0.0297429830279412\\
62	-0.0402794555215182\\
63	-0.0504310727801644\\
64	-0.0603229260736451\\
65	-0.0700150382559148\\
66	-0.0795339736665721\\
67	-0.0888890039187236\\
68	-0.100431353601506\\
69	-0.110975877473496\\
70	-0.120890884410267\\
71	-0.130372404850972\\
72	-0.139522923523005\\
73	-0.148394185707221\\
74	-0.157010462571295\\
75	-0.161816018157632\\
76	-0.167896235818783\\
77	-0.174526020273274\\
78	-0.181324394422291\\
79	-0.188089680178417\\
80	-0.19471367976463\\
81	-0.201136993069198\\
82	-0.20732575430733\\
83	-0.213259521613614\\
84	-0.218924973926207\\
85	-0.224312631555287\\
86	-0.229415263122681\\
87	-0.234226653693901\\
88	-0.238741519800768\\
89	-0.242955127128982\\
90	-0.249752779240954\\
91	-0.254936801913852\\
92	-0.259109481932212\\
93	-0.262590201291214\\
94	-0.265547819496892\\
95	-0.268071181017013\\
96	-0.270206668318991\\
97	-0.271978203381652\\
98	-0.273397901182008\\
99	-0.274471744300231\\
100	-0.275202605628669\\
};
\addlegendentry{v}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	0\\
2	-0.161680655065616\\
3	-0.247191965405639\\
4	-0.292726069809201\\
5	-0.3221445802988\\
6	-0.324203960120299\\
7	-0.324203970218803\\
8	-0.324203973129732\\
9	-0.32420397526987\\
10	-0.324203976726108\\
11	-0.324203977644951\\
12	-0.324203978185132\\
13	-0.324203978483872\\
14	-0.324203978642078\\
15	-0.324203740072803\\
16	-0.324203978138492\\
17	-0.324203978522645\\
18	-0.324203661432416\\
19	-0.324203804237188\\
20	-0.324203873659557\\
21	-0.324203912251722\\
22	-0.324203936104449\\
23	-0.324203951590514\\
24	-0.324203961720357\\
25	-0.324203968258315\\
26	-0.324203972389355\\
27	-0.324203974941278\\
28	-0.324203978109555\\
29	-0.324203978351329\\
30	-0.32420397850147\\
31	0.0513863172135708\\
32	0.16210198923802\\
33	0.162101971263516\\
34	0.162101966559462\\
35	0.162101960512762\\
36	0.162101952731778\\
37	0.162101942709097\\
38	0.162101929782529\\
39	0.162101913074666\\
40	0.162101989373046\\
41	0.162101989358861\\
42	0.162101989340027\\
43	0.162101989314362\\
44	0.162101989277922\\
45	0.162101989222998\\
46	0.1621019891338\\
47	0.162101988977103\\
48	0.16210198833143\\
49	0.162101987390957\\
50	0.162101985463763\\
51	0.162101981509989\\
52	0.162101973465523\\
53	0.162101957239027\\
54	0.162101923737667\\
55	0.0931365258568764\\
56	0.0524863140092813\\
57	0.0265013741541692\\
58	0.00813002411993019\\
59	-0.00626828622750331\\
60	-0.0185707427329436\\
61	-0.0297429830279412\\
62	-0.0402794555215182\\
63	-0.0504310727801644\\
64	-0.0603229260736451\\
65	-0.0700150382559148\\
66	-0.0795339736665721\\
67	-0.0888890039187236\\
68	-0.100431353601506\\
69	-0.110975877473496\\
70	-0.120890884410267\\
71	-0.130372404850972\\
72	-0.139522923523005\\
73	-0.148394185707221\\
74	-0.157010462571295\\
75	-0.161816018157632\\
76	-0.167896235818783\\
77	-0.174526020273274\\
78	-0.181324394422291\\
79	-0.188089680178417\\
80	-0.19471367976463\\
81	-0.201136993069198\\
82	-0.20732575430733\\
83	-0.213259521613614\\
84	-0.218924973926207\\
85	-0.224312631555287\\
86	-0.229415263122681\\
87	-0.234226653693901\\
88	-0.238741519800768\\
89	-0.242955127128982\\
90	-0.249752779240954\\
91	-0.254936801913852\\
92	-0.259109481932212\\
93	-0.262590201291214\\
94	-0.265547819496892\\
95	-0.268071181017013\\
96	-0.270206668318991\\
97	-0.271978203381652\\
98	-0.273397901182008\\
99	-0.274471744300231\\
100	-0.275202605628669\\
};
\addlegendentry{r}

\addplot [color=mycolor3]
  table[row sep=crcr]{%
1	-0.32420397881772\\
2	-0.324203978822229\\
3	-0.324203978828466\\
4	-0.324203978836056\\
5	-0.324203978843253\\
6	-0.324203978842642\\
7	-0.324203978839849\\
8	-0.324203978834392\\
9	-0.324203978825403\\
10	-0.324203978811692\\
11	-0.324203978791499\\
12	-0.324203978762273\\
13	-0.324203978720542\\
14	-0.324203978661947\\
15	-0.324203978581453\\
16	-0.324203978473736\\
17	-0.324203978333665\\
18	-0.324203978156826\\
19	-0.324203977940003\\
20	-0.32420397768155\\
21	-0.324203977381625\\
22	-0.324203977042247\\
23	-0.32420397666721\\
24	-0.324203976261852\\
25	-0.32420397583273\\
26	-0.324203975387235\\
27	-0.324203974933191\\
28	-0.324203974478466\\
29	-0.324203974030623\\
30	0.162101989317112\\
31	0.162101989322354\\
32	0.162101989327699\\
33	0.162101989333133\\
34	0.162101989338642\\
35	0.162101989344197\\
36	0.162101989349294\\
37	0.162101989354507\\
38	0.162101989359806\\
39	0.162101989365159\\
40	0.162101989370529\\
41	0.162101989375872\\
42	0.162101989381144\\
43	0.162101989386295\\
44	0.162101989391273\\
45	0.162101989396022\\
46	0.162101989400487\\
47	0.162101989404615\\
48	0.162101989408354\\
49	0.162101989411659\\
50	0.162101989414494\\
51	0.162101989416839\\
52	0.162101982845939\\
53	0.162101985605598\\
54	0.0197516801444962\\
55	0.00917834631732606\\
56	-0.00133716813198254\\
57	-0.0117844856600193\\
58	-0.0221532960255522\\
59	-0.0324333664644764\\
60	-0.042614551788306\\
61	-0.0526868043962439\\
62	-0.0626401841909603\\
63	-0.0724648683976596\\
64	-0.0821511612095226\\
65	-0.0916895034569802\\
66	-0.101070481934673\\
67	-0.110284838750594\\
68	-0.119323480446942\\
69	-0.128177486975623\\
70	-0.136838120501119\\
71	-0.145296834023719\\
72	-0.153545279814377\\
73	-0.161575317652907\\
74	-0.169379022861403\\
75	-0.176948694124936\\
76	-0.184276861091823\\
77	-0.19135629174596\\
78	-0.198179999543948\\
79	-0.204741250309971\\
80	-0.211033568881607\\
81	-0.217050745500034\\
82	-0.222786841938305\\
83	-0.228236197361658\\
84	-0.23339343391407\\
85	-0.238253462025547\\
86	-0.242811485434904\\
87	-0.247063005923097\\
88	-0.251003827752427\\
89	-0.254630061807248\\
90	-0.257938129432097\\
91	-0.260924765963466\\
92	-0.263587023951726\\
93	-0.26592227607002\\
94	-0.267928217707216\\
95	-0.269602869242327\\
96	-0.27094457799812\\
97	-0.271952019871938\\
98	-0.27262420064216\\
99	-0.272960456949034\\
100	-0.272960456949034\\
};
\addlegendentry{$\eta$}

\end{axis}

\begin{axis}[%
width=1.227\breite,
height=0.92\breite,
at={(-0.16\breite,-0.101\breite)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%

==> figures/Simulation_x.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\breite,
height=0.75\breite,
at={(0\breite,0\breite)},
scale only axis,
xmin=1,
xmax=100,
xlabel={time steps $t$},
ymin=-0.5,
ymax=1,
ylabel style={font=\color{white!15!black}},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black, legend pos = south east}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	0\\
2	0\\
3	0\\
4	0.007899328667822\\
5	0.0962227994774584\\
6	0.248017476706852\\
7	0.443014239915777\\
8	0.628092671866818\\
9	0.764995376313814\\
10	0.851159871976627\\
11	0.896980108082365\\
12	0.918173289783693\\
13	0.927006410222207\\
14	0.930417720865286\\
15	0.931663113759976\\
16	0.932099049518009\\
17	0.932246836506845\\
18	0.932295617249653\\
19	0.932311454174221\\
20	0.932316497968334\\
21	0.932317993586214\\
22	0.932318421670102\\
23	0.932318518402053\\
24	0.932318594441917\\
25	0.93231869085609\\
26	0.932318783545712\\
27	0.932318857333558\\
28	0.932318910459385\\
29	0.932318946728116\\
30	0.932318970816562\\
31	0.932318987180565\\
32	0.932318997752273\\
33	0.930289524584628\\
34	0.907484625240824\\
35	0.865890588796777\\
36	0.79656499086065\\
37	0.693096946638355\\
38	0.539035083893854\\
39	0.315057063747585\\
40	0.0656867833922573\\
41	-0.15495843649128\\
42	-0.310708677583323\\
43	-0.397611478837293\\
44	-0.438581101130539\\
45	-0.455784198129317\\
46	-0.462445394411426\\
47	-0.46487869122035\\
48	-0.465730225304973\\
49	-0.466018761496524\\
50	-0.466114148507325\\
51	-0.466145085076075\\
52	-0.466154968610476\\
53	-0.466158087273008\\
54	-0.466159058704154\\
55	-0.466159352146071\\
56	-0.466159426240934\\
57	-0.463328447666252\\
58	-0.430647633352469\\
59	-0.364831787103928\\
60	-0.275871403990953\\
61	-0.183655717953558\\
62	-0.104605765896837\\
63	-0.0420903632358335\\
64	0.00719582020410488\\
65	0.0476682523547058\\
66	0.0827642258380149\\
67	0.114693285746913\\
68	0.144743012977147\\
69	0.173619732562906\\
70	0.201808094563907\\
71	0.230560093256338\\
72	0.259850267617606\\
73	0.289509677900402\\
74	0.318806257049238\\
75	0.347237422714355\\
76	0.374663284179832\\
77	0.400958273441704\\
78	0.424607762839598\\
79	0.445980304146495\\
80	0.465509389005439\\
81	0.484377383217861\\
82	0.503293302592361\\
83	0.522355613257918\\
84	0.541373830335039\\
85	0.560109707732085\\
86	0.578371117834134\\
87	0.596025540539907\\
88	0.612986881040797\\
89	0.629199459051821\\
90	0.644625867530546\\
91	0.6592393649472\\
92	0.673160566784344\\
93	0.687671611499328\\
94	0.702482815787662\\
95	0.717229907027492\\
96	0.730929991063581\\
97	0.74299703620253\\
98	0.753352367050355\\
99	0.762154760050399\\
100	0.769598748340968\\
101	0.77583662845041\\
};
\addlegendentry{$\text{x}_\text{4}$}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	0.932319012147148\\
2	0.932319012160116\\
3	0.932319012178051\\
4	0.932319012199878\\
5	0.932319012220575\\
6	0.932319012218817\\
7	0.932319012210787\\
8	0.932319012195091\\
9	0.932319012169244\\
10	0.932319012129815\\
11	0.932319012071745\\
12	0.932319011987699\\
13	0.932319011867693\\
14	0.932319011699188\\
15	0.932319011467712\\
16	0.932319011157948\\
17	0.932319010755143\\
18	0.932319010246605\\
19	0.932319009623082\\
20	0.932319008879845\\
21	0.932319008017344\\
22	0.93231900704139\\
23	0.93231900596289\\
24	0.932319004797195\\
25	0.93231900356316\\
26	0.932319002282043\\
27	0.932319000976342\\
28	0.932318999668681\\
29	0.932318998380811\\
30	-0.466159505809733\\
31	-0.466159505824808\\
32	-0.466159505840178\\
33	-0.466159505855806\\
34	-0.466159505871647\\
35	-0.466159505887623\\
36	-0.466159505902279\\
37	-0.466159505917269\\
38	-0.466159505932509\\
39	-0.466159505947904\\
40	-0.466159505963345\\
41	-0.466159505978711\\
42	-0.466159505993872\\
43	-0.466159506008684\\
44	-0.466159506022998\\
45	-0.466159506036655\\
46	-0.466159506049497\\
47	-0.466159506061367\\
48	-0.466159506072119\\
49	-0.466159506081622\\
50	-0.466159506089776\\
51	-0.466159506096519\\
52	-0.466159487200468\\
53	-0.466159495136466\\
54	-0.0568002496074138\\
55	-0.0263943298997111\\
56	0.00384531761895967\\
57	0.0338888500667929\\
58	0.0637066181040259\\
59	0.0932691951932158\\
60	0.122547406639648\\
61	0.15151235838322\\
62	0.180135465513416\\
63	0.20838848050617\\
64	0.236243520961431\\
65	0.26367309740926\\
66	0.290650140131532\\
67	0.317148026047425\\
68	0.343140604942423\\
69	0.368602225279307\\
70	0.393507759512737\\
71	0.417832628887213\\
72	0.441552827693344\\
73	0.464644946958579\\
74	0.48708619754904\\
75	0.50885443265964\\
76	0.529928169670309\\
77	0.550286611346744\\
78	0.569909666364765\\
79	0.588777969138024\\
80	0.606872898929498\\
81	0.624176598227897\\
82	0.640671990370867\\
83	0.656342796397574\\
84	0.671173551114061\\
85	0.685149618355503\\
86	0.698257205430319\\
87	0.710483376731887\\
88	0.721816066504442\\
89	0.732244090750578\\
90	0.741757158268634\\
91	0.750345880809061\\
92	0.75800178233978\\
93	0.764717307411317\\
94	0.770485828613417\\
95	0.775301653115632\\
96	0.779160028285336\\
97	0.78205714637753\\
98	0.783990148291826\\
99	0.784957126393072\\
100	0.784957126393072\\
};
\addlegendentry{$\theta{}_\text{4}$}

\end{axis}

\begin{axis}[%
width=1.227\breite,
height=0.92\breite,
at={(-0.16\breite,-0.101\breite)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%

==> figures/simulation_221108/sim_alpha.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\breite,
height=\hohe,
at={(0\breite,0\hohe)},
scale only axis,
xmin=1,
xmax=1000,
ymin=-0,
ymax=1.05,
ylabel style={font=\color{white!15!black}},
ylabel={$\alpha$},
xlabel = {time steps $t$},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	1\\
2	0.268099414021203\\
3	0.0222808280331037\\
4	0.055231602705569\\
5	0.0641439828092656\\
6	0.152844016959442\\
7	0.187332373180288\\
8	0.0881022651737062\\
9	0.162190695933378\\
10	0.275068619946075\\
11	0.23347481716878\\
12	0.36715200597135\\
13	0.58183125901028\\
14	1\\
15	1\\
16	1\\
17	1\\
18	1\\
19	1\\
20	1\\
21	1\\
22	1\\
23	1\\
24	1\\
25	1\\
26	1\\
27	1\\
28	1\\
29	1\\
30	1\\
31	1\\
32	1\\
33	1\\
34	1\\
35	1\\
36	1\\
37	1\\
38	1\\
39	1\\
40	1\\
41	1\\
42	1\\
43	1\\
44	1\\
45	1\\
46	1\\
47	1\\
48	1\\
49	1\\
50	1\\
51	1\\
52	1\\
53	1\\
54	1\\
55	1\\
56	1\\
57	1\\
58	1\\
59	1\\
60	1\\
61	1\\
62	1\\
63	1\\
64	1\\
65	1\\
66	1\\
67	1\\
68	1\\
69	1\\
70	1\\
71	1\\
72	1\\
73	1\\
74	1\\
75	0.05008824711578\\
76	0.00396256554173924\\
77	0.0070447696228797\\
78	0.0297490144569066\\
79	0.0181219192804338\\
80	0.0132562935883582\\
81	0.0423909361045132\\
82	0.0360742849129307\\
83	0.0294382272201457\\
84	0.0679149207544603\\
85	0.0716051157222681\\
86	0.0665226039147448\\
87	0.12583514114677\\
88	0.135570409368721\\
89	0.0662450968138932\\
90	0.134805696857301\\
91	0.179208517348244\\
92	0.149733451010093\\
93	0.202253436683584\\
94	0.262287730323439\\
95	0.342791721955367\\
96	0.472494159479638\\
97	1\\
98	1\\
99	1\\
100	1\\
101	1\\
102	1\\
103	1\\
104	1\\
105	1\\
106	1\\
107	1\\
108	1\\
109	1\\
110	1\\
111	1\\
112	1\\
113	1\\
114	1\\
115	1\\
116	1\\
117	1\\
118	1\\
119	1\\
120	1\\
121	1\\
122	1\\
123	1\\
124	1\\
125	1\\
126	1\\
127	1\\
128	1\\
129	1\\
130	1\\
131	1\\
132	1\\
133	1\\
134	1\\
135	1\\
136	1\\
137	1\\
138	1\\
139	1\\
140	1\\
141	1\\
142	1\\
143	1\\
144	1\\
145	1\\
146	1\\
147	1\\
148	0.445343121989721\\
149	0.0277552172327304\\
150	0.0583824063311358\\
151	0.062598590289717\\
152	0.147072813122136\\
153	0.177673196319323\\
154	0.0814741786779676\\
155	0.146559916099269\\
156	0.248712033954426\\
157	0.199871190683457\\
158	0.303930403330308\\
159	0.432998578477012\\
160	0.804039674429897\\
161	1\\
162	1\\
163	1\\
164	1\\
165	1\\
166	1\\
167	1\\
168	1\\
169	1\\
170	1\\
171	1\\
172	1\\
173	1\\
174	1\\
175	1\\
176	1\\
177	1\\
178	1\\
179	1\\
180	1\\
181	1\\
182	1\\
183	1\\
184	1\\
185	1\\
186	1\\
187	1\\
188	1\\
189	1\\
190	1\\
191	1\\
192	1\\
193	1\\
194	1\\
195	1\\
196	1\\
197	1\\
198	1\\
199	1\\
200	1\\
201	1\\
202	1\\
203	1\\
204	1\\
205	1\\
206	1\\
207	1\\
208	1\\
209	1\\
210	1\\
211	1\\
212	1\\
213	1\\
214	1\\
215	1\\
216	1\\
217	1\\
218	1\\
219	1\\
220	1\\
221	1\\
222	1\\
223	1\\
224	1\\
225	1\\
226	1\\
227	1\\
228	1\\
229	1\\
230	1\\
231	1\\
232	1\\
233	1\\
234	1\\
235	1\\
236	1\\
237	0.187630692485797\\
238	0.0163779471860286\\
239	0.0291144854877698\\
240	0.124227370317033\\
241	0.05302276486794\\
242	0.0376953332926462\\
243	0.086216451882474\\
244	0.091360275756311\\
245	0.063258899281009\\
246	0.0946533103436522\\
247	0.0999323588804932\\
248	0.108462723632615\\
249	0.111371520100296\\
250	0.142316865958525\\
251	0.14861498307339\\
252	0.184206091128433\\
253	0.212761624521955\\
254	0.285388064478793\\
255	0.370747937437589\\
256	0.617898988086577\\
257	1\\
258	1\\
259	1\\
260	1\\
261	1\\
262	1\\
263	1\\
264	1\\
265	1\\
266	1\\
267	1\\
268	1\\
269	1\\
270	1\\
271	1\\
272	1\\
273	1\\
274	1\\
275	1\\
276	1\\
277	1\\
278	1\\
279	1\\
280	1\\
281	1\\
282	1\\
283	1\\
284	1\\
285	1\\
286	1\\
287	1\\
288	1\\
289	1\\
290	1\\
291	1\\
292	1\\
293	1\\
294	1\\
295	1\\
296	1\\
297	1\\
298	1\\
299	1\\
300	1\\
301	1\\
302	1\\
303	1\\
304	1\\
305	0.208257794908785\\
306	0.018338145295921\\
307	0.0326620430836053\\
308	0.138698781369778\\
309	0.0993005107316414\\
310	0.076980133568898\\
311	0.0681458763719052\\
312	0.14931341708041\\
313	0.141982904841885\\
314	0.0947257091753828\\
315	0.206533766845337\\
316	0.189590776468117\\
317	0.269096128323216\\
318	0.309693574077681\\
319	0.580857500854277\\
320	1\\
321	1\\
322	1\\
323	1\\
324	1\\
325	1\\
326	1\\
327	1\\
328	1\\
329	1\\
330	1\\
331	1\\
332	1\\
333	1\\
334	1\\
335	1\\
336	1\\
337	1\\
338	1\\
339	1\\
340	1\\
341	1\\
342	1\\
343	1\\
344	1\\
345	1\\
346	1\\
347	1\\
348	1\\
349	1\\
350	1\\
351	1\\
352	1\\
353	1\\
354	1\\
355	1\\
356	1\\
357	1\\
358	1\\
359	1\\
360	1\\
361	1\\
362	1\\
363	1\\
364	1\\
365	1\\
366	1\\
367	1\\
368	1\\
369	1\\
370	1\\
371	1\\
372	1\\
373	1\\
374	1\\
375	1\\
376	1\\
377	1\\
378	1\\
379	1\\
380	1\\
381	1\\
382	1\\
383	1\\
384	1\\
385	1\\
386	1\\
387	1\\
388	1\\
389	1\\
390	1\\
391	1\\
392	1\\
393	1\\
394	1\\
395	1\\
396	1\\
397	1\\
398	1\\
399	1\\
400	1\\
401	1\\
402	1\\
403	1\\
404	1\\
405	1\\
406	1\\
407	1\\
408	1\\
409	1\\
410	1\\
411	1\\
412	1\\
413	1\\
414	1\\
415	1\\
416	1\\
417	1\\
418	1\\
419	1\\
420	1\\
421	1\\
422	1\\
423	1\\
424	1\\
425	1\\
426	1\\
427	1\\
428	1\\
429	1\\
430	1\\
431	1\\
432	1\\
433	1\\
434	1\\
435	1\\
436	1\\
437	1\\
438	1\\
439	1\\
440	1\\
441	1\\
442	1\\
443	1\\
444	1\\
445	1\\
446	1\\
447	1\\
448	1\\
449	1\\
450	1\\
451	1\\
452	1\\
453	1\\
454	1\\
455	1\\
456	1\\
457	1\\
458	1\\
459	1\\
460	1\\
461	1\\
462	1\\
463	1\\
464	1\\
465	1\\
466	1\\
467	1\\
468	1\\
469	1\\
470	1\\
471	1\\
472	1\\
473	1\\
474	1\\
475	1\\
476	1\\
477	1\\
478	1\\
479	1\\
480	1\\
481	1\\
482	1\\
483	1\\
484	1\\
485	1\\
486	1\\
487	1\\
488	1\\
489	1\\
490	1\\
491	1\\
492	1\\
493	1\\
494	1\\
495	1\\
496	1\\
497	1\\
498	1\\
499	1\\
500	1\\
501	1\\
502	1\\
503	1\\
504	1\\
505	1\\
506	1\\
507	1\\
508	1\\
509	1\\
510	1\\
511	1\\
512	1\\
513	1\\
514	1\\
515	1\\
516	1\\
517	1\\
518	1\\
519	1\\
520	1\\
521	1\\
522	1\\
523	1\\
524	1\\
525	1\\
526	1\\
527	1\\
528	1\\
529	1\\
530	1\\
531	1\\
532	1\\
533	1\\
534	1\\
535	1\\
536	1\\
537	1\\
538	1\\
539	1\\
540	1\\
541	1\\
542	1\\
543	1\\
544	1\\
545	1\\
546	1\\
547	1\\
548	1\\
549	1\\
550	1\\
551	1\\
552	1\\
553	1\\
554	1\\
555	1\\
556	1\\
557	1\\
558	1\\
559	1\\
560	1\\
561	1\\
562	1\\
563	1\\
564	1\\
565	1\\
566	1\\
567	1\\
568	1\\
569	1\\
570	1\\
571	1\\
572	1\\
573	1\\
574	1\\
575	1\\
576	1\\
577	1\\
578	1\\
579	1\\
580	1\\
581	1\\
582	1\\
583	1\\
584	1\\
585	1\\
586	1\\
587	1\\
588	1\\
589	1\\
590	1\\
591	1\\
592	1\\
593	1\\
594	1\\
595	1\\
596	1\\
597	1\\
598	1\\
599	1\\
600	1\\
601	1\\
602	1\\
603	1\\
604	1\\
605	1\\
606	1\\
607	1\\
608	1\\
609	1\\
610	1\\
611	1\\
612	1\\
613	1\\
614	1\\
615	1\\
616	1\\
617	1\\
618	1\\
619	1\\
620	1\\
621	1\\
622	1\\
623	1\\
624	1\\
625	1\\
626	1\\
627	1\\
628	1\\
629	1\\
630	1\\
631	1\\
632	1\\
633	1\\
634	1\\
635	1\\
636	1\\
637	1\\
638	1\\
639	1\\
640	1\\
641	1\\
642	1\\
643	1\\
644	1\\
645	1\\
646	1\\
647	1\\
648	1\\
649	1\\
650	1\\
651	1\\
652	1\\
653	1\\
654	1\\
655	1\\
656	1\\
657	1\\
658	1\\
659	1\\
660	1\\
661	1\\
662	1\\
663	1\\
664	1\\
665	1\\
666	1\\
667	1\\
668	1\\
669	1\\
670	1\\
671	1\\
672	1\\
673	1\\
674	1\\
675	1\\
676	1\\
677	1\\
678	1\\
679	1\\
680	1\\
681	1\\
682	1\\
683	1\\
684	1\\
685	1\\
686	1\\
687	1\\
688	1\\
689	1\\
690	1\\
691	1\\
692	1\\
693	1\\
694	1\\
695	1\\
696	1\\
697	1\\
698	1\\
699	1\\
700	1\\
701	1\\
702	1\\
703	1\\
704	1\\
705	1\\
706	1\\
707	1\\
708	1\\
709	1\\
710	1\\
711	1\\
712	1\\
713	1\\
714	1\\
715	1\\
716	1\\
717	1\\
718	1\\
719	1\\
720	1\\
721	1\\
722	1\\
723	1\\
724	1\\
725	1\\
726	1\\
727	1\\
728	1\\
729	1\\
730	1\\
731	1\\
732	1\\
733	1\\
734	1\\
735	1\\
736	1\\
737	1\\
738	1\\
739	1\\
740	1\\
741	1\\
742	1\\
743	1\\
744	1\\
745	1\\
746	1\\
747	1\\
748	1\\
749	1\\
750	1\\
751	1\\
752	1\\
753	1\\
754	1\\
755	1\\
756	1\\
757	1\\
758	1\\
759	1\\
760	1\\
761	1\\
762	1\\
763	1\\
764	1\\
765	1\\
766	1\\
767	1\\
768	1\\
769	1\\
770	1\\
771	1\\
772	1\\
773	1\\
774	1\\
775	1\\
776	1\\
777	1\\
778	1\\
779	1\\
780	1\\
781	1\\
782	1\\
783	1\\
784	1\\
785	1\\
786	1\\
787	1\\
788	1\\
789	1\\
790	1\\
791	1\\
792	1\\
793	1\\
794	1\\
795	1\\
796	1\\
797	1\\
798	1\\
799	1\\
800	1\\
801	1\\
802	1\\
803	1\\
804	1\\
805	1\\
806	1\\
807	1\\
808	1\\
809	1\\
810	1\\
811	1\\
812	1\\
813	1\\
814	1\\
815	1\\
816	1\\
817	1\\
818	1\\
819	1\\
820	1\\
821	1\\
822	1\\
823	1\\
824	1\\
825	1\\
826	1\\
827	1\\
828	1\\
829	1\\
830	1\\
831	1\\
832	1\\
833	1\\
834	1\\
835	1\\
836	1\\
837	1\\
838	1\\
839	1\\
840	1\\
841	1\\
842	1\\
843	1\\
844	1\\
845	1\\
846	0.404043321931749\\
847	0.0241493298069271\\
848	0.0509841115700738\\
849	0.0541415338589255\\
850	0.126928102413438\\
851	0.150276282610776\\
852	0.0666270680404297\\
853	0.117574483442052\\
854	0.194389656804231\\
855	0.145038335337351\\
856	0.207373265191754\\
857	0.259257904081683\\
858	0.37110066402375\\
859	0.489020307607751\\
860	1\\
861	1\\
862	1\\
863	1\\
864	1\\
865	1\\
866	1\\
867	1\\
868	1\\
869	1\\
870	1\\
871	1\\
872	1\\
873	1\\
874	1\\
875	1\\
876	1\\
877	1\\
878	1\\
879	0.169579695116548\\
880	0.0144870901700935\\
881	0.0257837956906926\\
882	0.1091288990757\\
883	0.0750646124568899\\
884	0.0569967082827336\\
885	0.152062708026661\\
886	0.057721911960857\\
887	0.112250670243866\\
888	0.138082120946799\\
889	0.15007042733758\\
890	0.14461984278788\\
891	0.219296495045449\\
892	0.241511930020478\\
893	0.343869734254143\\
894	0.487674424739664\\
895	1\\
896	1\\
897	1\\
898	1\\
899	1\\
900	1\\
901	1\\
902	1\\
903	1\\
904	1\\
905	1\\
906	1\\
907	1\\
908	1\\
909	1\\
910	1\\
911	1\\
912	1\\
913	1\\
914	1\\
915	1\\
916	1\\
917	1\\
918	1\\
919	1\\
920	1\\
921	1\\
922	1\\
923	1\\
924	1\\
925	1\\
926	1\\
927	1\\
928	1\\
929	1\\
930	1\\
931	1\\
932	1\\
933	1\\
934	1\\
935	1\\
936	1\\
937	1\\
938	1\\
939	1\\
940	1\\
941	1\\
942	1\\
943	1\\
944	1\\
945	1\\
946	1\\
947	1\\
948	1\\
949	1\\
950	1\\
951	1\\
952	1\\
953	1\\
954	1\\
955	1\\
956	1\\
957	1\\
958	1\\
959	1\\
960	1\\
961	1\\
962	1\\
963	1\\
964	1\\
965	1\\
966	1\\
967	1\\
968	1\\
969	1\\
970	1\\
971	1\\
972	1\\
973	1\\
974	1\\
975	1\\
976	1\\
977	1\\
978	1\\
979	1\\
980	1\\
981	1\\
982	1\\
983	1\\
984	1\\
985	1\\
986	1\\
987	1\\
988	1\\
989	1\\
990	1\\
991	1\\
992	1\\
993	1\\
994	1\\
995	1\\
996	1\\
997	1\\
998	1\\
999	1\\
1000	1\\
};

\end{axis}

\begin{axis}[%
width=1.227\breite,
height=1.227\hohe,
at={(-0.16\breite,-0.135\hohe)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
